Centralized Volatility Reduction for Electricity Markets

Increased penetration of wind energy will make electricity market prices more volatile. As a result, market participants will bear increased financial risks, which impact investment decisions and in turn, makes it harder to achieve sustainable energy goals. As a remedy, in this paper, we propose an insurance market that complements any wholesale market design. Our mechanism can be run by any suitable financial entity such as an independent system operator, with the aim of reducing the financial impacts of volatile prices. We provide theoretical guarantees, analytically characterize the outcomes over a copperplate power system example, and numerically explore the same for a modified IEEE 14-bus test system.

==> conclusion.tex <==
%!TEX root = OptionPaper.tex
\section{Conclusions}
\label{sec:conc}

This paper has proposed a design of a centralized cash-settled options market that can be implemented in realistic scenarios. An attractive feature of the proposed design is that it can be applied to any existing electricity market, making its implementation less complex. We have shown the existence of optimal solutions for the centralized mechanism, provided theoretical guarantees on total variances, and provided participant-specific conditions to guarantee strict volatility reduction. We have also conducted extensive numerical experiments on both the stylized example and the IEEE 14 bus test system, with considerations related to financial transmission rights and the effect of risk-aversion. Future works include: multi-period considerations, joint optimization for market participants, and theoretical studies for risk-averse market participants.



==> motivation.tex <==
%!TEX root = OptionPaper.tex


\subsection{A copperplate power system example} \label{sec:motivate}

We present here a stylized single-bus power system example (adopted from \cite{bose}) and illustrate how a bilateral trade (a cash-settled call option) can reduce the volatility in payments of market participants, and even mitigate the risks of financial losses for some. 
%, which generalizes the bilateral trade to all market participants and improves on the benefits.
% adopted for electricity markets with deep renewable penetration. 


Consider a power system with two dispatchable generators and a single variable renewable wind power producer serving a demand $d$. In this example, $ \Gset := \{ B, P \}, \quad \text{and} \quad \mathfrak{R} : = \{ W \}$,
where $B$ is a base-load generator, $P$ is a peaker power plant, and $W$ is a wind power producer. 

Let $x_B^{\text{cap}} = x_P^{\text{cap}} = \infty, \quad \text{and} \quad \ell_B = 0, \ \ell_P= \infty.$
Therefore, $B$ and $P$ have unlimited generation capacities. $B$ does not have the flexibility to alter its output in realtime from its forward set-point. In contrast, $P$ has no ramping limitations. Let $B$ and $P$ have linear costs of production. $B$ has a unit marginal cost, and $P$ has a marginal cost of $1/{\rho}$, where  $\rho \in (0,1]$, i.e., $P$ is more expensive than $B$.


%\begin{figure}
%\begin{center}
%\includegraphics[scale=0.65]{StylizedExample}    % The printed column width is 8.4 cm.
%\caption{The stylized power system example}
%\label{fig:StylizedExample}
%\end{center}
%\end{figure}%The aggregate demand $d$ is inflexible and known a day in advance. Assume $d \geq \mu + \sqrt{3} \sigma$.

Encode the uncertainty in available wind in the set
$$ \Omega := [\mu - \sqrt{3}\sigma, \mu + \sqrt{3}\sigma] \subset \Rset_+,$$
and take $\prob$ to be the uniform distribution over $\Omega$. That is, available wind is uniform with mean $\mu$ and variance $\sigma^2$. Scenario $\omega \in \Omega$ defines an available wind capacity of $\overline{x}_r^\omega = \omega$. Further, assume that $W$ produces power at zero cost, and fixed demand $d \geq \mu + \sqrt{3} \sigma$. 
%An illustration of this example is shown in Figure \ref{fig:StylizedExample}.

This stylized example is a caricature of electricity markets with deepening penetration of variable renewable wind supply. Base-load generators, specifically nuclear power plants, have limited ramping capabilities. Natural gas based peakers can quickly ramp their power outputs. Utilizing them to balance variability can be costly. Finally, (aggregated) demand is largely inflexible but predictable. In the remainder of this section, we analyze the effect of a bilateral call option on the market outcome for this example. 


%\subsection{Market outcome}

The benchmark dispatch model yields the following forward and realtime dispatch decisions $X^*$, $x^{*, \omega}$, and the forward and realtime prices $P^*, p^{*, \omega}$, respectively. See \cite{bose} for the calculations. \footnote{{\color{black} This dispatch is not optimal in the sense of minimizing the expected aggregate cost of production. It is the solution to the benchmark electricity market model in the previous section applied to the copperplate power system example.}}
\begin{itemize}
\item $X_B^* = d - \mu, \ X_P^* = 0, \ X_W^* = \mu$.
\item $x_B^{\omega,*} = d - \mu, \ x_W^{\omega,*} = \min\{\omega, \mu\}, \ x_P^{\omega,*} = (\mu - \omega)^+$.
\item $P^* = 1, \ p^{\omega,*} = (1/\rho) \ind{\omega \in \[ \mu-\sqrt{3}\sigma, \mu \]}$. 
\end{itemize}

% \bose{Do you need this bit here? You have already stated that in the end of Section II. Maybe make it into a footnote.} 
The above dispatch and the prices yield the following payments of the market participants in scenario $\omega$:
%
\begin{align*}
\small{
\pi_B^\omega = d-\mu, 
\; \; \pi_P^\omega = (\mu-\omega)^+/\rho, \; \;
\pi_W^\omega = \mu - ( \mu - \omega)^+/\rho. 
}
%\pi_D(\omega) = c_B d.
\end{align*}
It is straightforward to conclude from the above payments that $W$ incurs a financial loss for scenarios in
\begin{align}
\Omega_0^- := \left[ \mu - \sqrt{3} \sigma, \ \mu (1 - \rho) \right).
\label{eq:Omega0}
\end{align}
when $\rho < \sqrt{3} \frac{\sigma}{\mu}$. In what follows, we consider a bilateral call option trade between $P$ and $W$, and demonstrate that the option trade reduces the volatilities of $P$ and $W$'s payments, and further shrinks the scenarios in $\Omega_0^-$ where $W$ incurs a financial loss.

%Next, we consider a bilateral cash-settled option between $P$ and $W$. We will show that  such an option can reduce the volatility of the payments to $W$ and $P$. Also of interest is $W$'s payment, when $\rho < \sqrt{3} \frac{\sigma}{\mu}$ and the realized available wind $\omega$ is in $\Omega_0^-$, where
%\begin{align}
%\Omega_0^- := \lb \omega \ : \ \mu - \sqrt{3} \sigma \leq \omega < \mu (1 - \rho) \rb.
%\label{eq:Omega0}
%\end{align}
%For such a scenario $\omega$, we have $\pi_W^\omega < 0$. That is, $W$ incurs a loss for each $\omega \in \Omega_0^-$. As we will illustrate, $W$ can avoid incurring such a loss in a subset of the scenarios by trading in an option with $P$. 

%------------------------------------------
%\subsection{Adding call option trade between $W$ and $P$}\label{sec:motivate.bilateral}

 In \cite{IFAC}, a bilateral option trade between $P$ and $W$ was modeled as a robust Stackelberg game (see \cite{basar}) $\Gcal$ as follows. Right after the day ahead market is settled at $t=0$, $P$ announces an option price $q \in \Rset_+$ and a strike price $K \in \Rset_+$ for the call option it sells. Then, $W$ responds by purchasing $\Delta \in \Rset_+$ options. This option entitles $W$ to a cash payment of $\left( p^{\omega,*} - K \right)^+\Delta$ from $P$ in scenario $\omega$. The option costs $W$ a fee of $q\Delta$. It was shown in \cite{IFAC} that over all nontrivial equilibria $(q^*,K^*,\Delta^*)$ with $\Delta^* = \sqrt{3} \sigma$, it follows that
 $$
{\sf var}\left[\Pi^\omega_i(q^*, K^*, \sqrt{3}\sigma)\right]
- {\sf var}\left[\pi^\omega_i\right] 
= - \frac{3}{2}{{q^*K^*}}{\sigma^2}  < 0,
$$
where $2q^* + K^* = \rho^{-1}$. 

%Assume that there is an exogenously defined cap of $\sqrt{3}\sigma$ on the amount of option $W$ can buy from $P$. The cap equals the maximum shortfall that $W$ can incur from the electricity market in real time.
%
%When they agree on the trade triple $\(q,K,\Delta\)$, the total payments to $P$ and $W$ in scenario $\omega$ are given by
%\begin{align}
%\begin{aligned}
%\Pi^\omega_W(q, K, \Delta) &:= \pi_W^\omega - q \Delta + \left( p^{\omega,*} - K \right)^+\Delta,\\
%\Pi^\omega_P(q, K, \Delta) &:= \pi_P^\omega + q\Delta - \left( p^{\omega,*} - K \right)^+\Delta, 
%\end{aligned}
%\label{eq:Pi}
%\end{align}
%respectively. In each expression, the first term is the payment from the electricity market, and the other two terms come from the option trade.
%% where $(q^*, K^* , \Delta^*)$ comprises a Nash equilibrium of $\Gcal$. Let ${\sf var}[x(\omega)]$ denote the variance of a real valued map $x:\Omega \to \Rset$.
%Assume that $W$ is risk-neutral and has the correct conjectures on the real-time prices. Then, the perceived payoff for $W$ in the forward stage is given by $\E \left[\Pi^\omega_W(q, K, \Delta)\right]$.
%% If $W$ believes in a different price distribution, the perceived payoff for $W$ can be modified accordingly. Moreover, if $W$ is risk-averse, one can replace $\E$ with a suitable risk-functional. Similar considerations extend to the perceived payoff for $P$. The effect of risk-aversion will be discussed later in the paper.



%The possible outcomes of the option trade are identified as the set of Stackelberg equilibria (SE) of $\Gcal$. 
%{\color{black}
%\begin{definition} We say $(q^*, K^*, \Delta^*(q^*, K^*))$ constitutes a Stackelberg equilibrium, if 
%$$\E\left[\Pi_P^\omega(q^*, K^*, \Delta^*(q^*, K^*))\right] \geq \E\left[\Pi_P^\omega(q, K, \Delta^*(q, K))\right],$$
%where $\Delta^*:\Rset^2_+\rightarrow[0,\sqrt{3}\sigma]$ is the best response of $W$. Given $(q,K)$, the best response $\Delta^*$ satisfies $$\E\left[\Pi_W^\omega(q, K, \Delta^*(q, K))\right] \geq \E\left[\Pi_W^\omega(q, K, \Delta(q, K))\right].$$
%\end{definition}
%
%Stackelberg games are sequential games in which the leader(s) acts first, and then the follower(s) responds. In the determination of their decisions, leaders anticipate how followers would respond. In our game, $P$ is the leader and chooses $(q,K)$, given the best response $\Delta^*(q,K)$ by $W$ to the prices $(q,K)$. We have the following result.}%
%%
%\begin{proposition}
%\label{prop:bilat}
%The Stackelberg equilibria of $\Gcal$ are given by $(q^*,K^*) \in \Rset^2_+$ and $\Delta^*: \Rset^2_+ \to [0, \sqrt{3} \sigma]$ that satisfy one of the following conditions:
%\begin{itemize}
%\item[(i)] $2q^* + K^* > \rho^{-1}$, and $\Delta^* = 0$,
%\item[(ii)] $2q^* + K^* = \rho^{-1}$, and $\Delta^*\in[0, \sqrt{3} \sigma]$.
%\end{itemize}
%Over all equilibria with $\Delta^* = \sqrt{3} \sigma$,
% $$
%{\sf var}\left[\Pi^\omega_i(q^*, K^*, \sqrt{3}\sigma)\right]
%- {\sf var}\left[\pi^\omega_i\right] 
%= - \frac{3}{2}{{q^*K^*}}{\sigma^2}  < 0
%$$
%for each $i = W, P$.
%
%%\noindent Furthermore,  $\Pi_W^{\omega,*}(q^*, K^*, \Delta^*)< 0$ for $\omega \in \Omega^{-}$, defined as
%%$$\Omega^-:=\left[ \mu - \sqrt{3} \sigma, \  \mu (1 - \rho)-{\rho} q^*\Delta^* \right)$$
%%when $\rho < \sqrt{3} \frac{\sigma}{\mu}$.
%\end{proposition}
%%



%\khaled{Prop. and discussion are updated}
%%
%\begin{proposition}
%\label{prop:bilat}
%The Stackelberg equilibria of $\Gcal$ are given by 
%$\Ncal_1 \cup \Ncal_2$, where
%\begin{align*}
%\Ncal_1 &:= \left\{ (q, K, \Delta) \ \vert \ (q,K) \in \Rset_+^2, \ \Delta:\Rset^2_+ \to [0, \sqrt{3}\sigma], \right.\\
%&\qquad\quad \left. 2q + K > 1/\rho , \ \Delta(q', K') = 0 \ \forall \ (q', K') \in\Rset^2_+  \right\},\\ 
%%\Ncal_1 &:= \left\{ (q, K, \Delta(q,K)) \in \Rset_3^+ \ : \ q + K > 1/\rho , \ \Delta = 0 \right\},\\ 
%\Ncal_2 &:= \left\{ (q, K, \Delta) \ \vert \ (q,K) \in \Rset_+^2, \ \Delta:\Rset^2_+ \to [0, \sqrt{3}\sigma], \right.\\ &\qquad\quad \left. 2q + K = 1/\rho \right\}.
%\end{align*}
%Moreover, for $(q^*>0, K^*>0, \Delta^*(q^*, K^*)=\sqrt{3} \sigma) \in \Ncal_2$, the variances of the payments satisfy
%$$
%{\sf var}\left[\Pi^\omega_i(q^*, K^*, \Delta^*(q^*, K^*))\right]
%- {\sf var}\left[\pi^\omega_i\right] 
%= - 3{{q^*K^*}}{\sigma^2} /2< 0,
%$$
%for each $i \in \lb W, P \rb$.
%\end{proposition}
%%
%%
%\begin{prop}
%\label{prop:bilat}
%If $\frac{1}{\rho}c_B<q+K$, then 
%$$\frac{1}{\rho} c_B<q^*+K^*,\ \ \text{ and } \ \ \Delta^* = 0,$$
%define the Nash equilibria $(q^*, K^*, \Delta^*) \in \Rset^3_+$ of the game $\Gcal$. 
%Otherwise, the Nash equilibria are given by 
%\begin{equation}2q^* + K^* = \frac{1}{\rho} c_B, \ \ \text{ and } \ \ \Delta^* = \sqrt{3}\sigma.\label{NE} \end{equation}
%Moreover, any Nash equilibrium in (\ref{NE}) satisfies
%\begin{align*}
%{\sf var}[\Pi^\omega_W]
%- {\sf var}[\pi^\omega_W] 
%= 
%{\sf var}[\Pi^\omega_P] -
%{\sf var}[\pi_P^\omega]  \\
%= -\frac{q^*c_B}{2\rho}(2\mu(\mu-\sqrt{3}\sigma)+\frac{3\sigma^2}{2}) < 0.
%\end{align*}
%
%\begin{align*}
%[\Pi^\omega_W]
%- [\pi^\omega_W] 
%= 
%-([\Pi^\omega_P] -
%[\pi_P^\omega])  \\
%= \left\{ \begin{array} {ll}q^*\sqrt{3}\sigma\,\,&\,\, \text{if}\,\, \omega < \mu,\\ -q^*\sqrt{3}\sigma\,\, &\,\, \text{if}\,\, \omega \geq \mu. \end{array}\right.
%\end{align*}
%\end{prop}
%%
%Proof of this Proposition can be found in \cite{arxiv}.

%The first kind of equilibria with $\Delta^* = 0$ describes the degenerate case, where no trading occurs. $P$ and $W$ engage in trading at the second kind of equilibria, where the option/strike prices satisfy $ 2q^* +K^* = \rho^{-1}$. While we explicitly state the variance reduction only for the case $\Delta^*=\sqrt{3}\sigma$, the variance reduces more generally for any $\Delta^* \neq 0$, as our proof reveals. Lower $\rho$ implies a costlier peaker plant, that in turn indicates a higher price variation in the realtime market. Then, one would expect the potential for volatility reduction (through option trade) to grow with lower $\rho$. Notice how Proposition \ref{prop:bilat} reveals the same -- smaller $\rho$ leads to equilibria with higher option and strike prices, owing to the relation $2q^* +K^* = \rho^{-1}$, allowing the reduction $\frac{3}{2}{{q^*K^*}}{\sigma^2}$ to increase. The reduction in variance also increases with $\sigma^2$. Again, participants stand to gain more (in terms of volatility reduction) from the option trade as the available wind becomes more uncertain.

%Finally, recall that $W$ suffers a financial loss in the energy market whenever $\rho < \sqrt{3} \frac{\sigma}{\mu}$ and $\omega \in \Omega_0^-$ as defined in \eqref{eq:Omega0}. Here,  $\Pi_W^{\omega,*}(q^*, K^*, \Delta^*)< 0$ for $\omega \in \Omega^{-}$, where $$\Omega^-:=\left[ \mu - \sqrt{3} \sigma, \  \mu (1 - \rho)-{\rho} q^*\Delta^* \right).$$ With the bilateral option trade, $W$ suffers a loss only for scenarios in $\Omega^- \subset \Omega_0^{-}$, i.e., $W$ is less exposed to negative payments with option trade. 
%\subsection{Limitations of bilateral trading} 
%{\color{black}The former analysis on the copperplate power system example reveals the benefits of a bilateral trade in call options as an instrument to reduce payment volatilities. In a wholesale market with a collection of dispatchable generators $\Gfk$ and variable generators $\Rfk$, one can conceive of $\lvert \Gfk \rvert \cdot \lvert \Rfk \rvert $ bilateral option trades. It is difficult to convene and settle a large number of bilateral trades on a regular basis. Financial exchanges provide an alternative that typically seek to maximize the surplus from trading (options and other financial derivatives) with a collection of market participants.
%%Large volumes of options can be cleared via exchanges, which usually maximize the surplus of traders. 
%In this paper, we take an alternate route, and propose a centralized clearing mechanism for both buyers and sellers of call options with a goal to reduce payment volatilities in electricity markets. Next, we describe our options market design and highlight its differences from a traditional exchange.
}
%is to propose a mechanism that can clear the options in a way that guarantees volatility reductions, and hence our approach is different from designing a traditional exchange. We discuss our options market next.}

%----------------------------------------------------------------------------




%For convenience, define the additional notation
%\begin{align*}
%\Pi_P (\omega) &:= \pi_P(\omega) + V_P(\omega), \\
%\Pi_W (\omega) &:= \pi_W(\omega) + V_W(\omega),
%\end{align*}
%to denote the total payments to $P$ and $W$ in scenario $\omega$. 




%The following result 


%The wind power producer is exposed to the risk of receiving negative payments with the certainty equivalent dispatch under high uncertainty. This is a situation of interest in our analysis because it reflects high volatility in payments under uncertainty. The availability of the swing option allows the wind power producer to acquire more energy in real-time by exercising his option and reduce his losses. 

%The peaker power plant with the certainty equivalent dispatch might not be needed when there is a high availability of wind power (since it is cheaper to use the wind power plant instead of activating a more costly peaker generator). But, with a bilateral swing option, in the forward stage he can be paid for the flexibility $\Delta$ he sells, and dependent on the realization of the scenario $\omega$, if the availability of wind is high, then the peaker generator is better off, and receives $q\Delta$ instead of zero. In the case when there's a low availability of wind power supply, if the wind producer exercises his right, he will be pay the peaker plant $K\delta(\omega)$ in real-time. 



%The total payment to the wind power producer and the peaker power plant is the sum of his payment in the certainty equivalent dispatch and his valuation of the swing option. Precisely, 
%\begin{eqnarray*} 
%\pi^{total}_W&:=&\pi_W+V_W\\
%&=& c_B\mu+p^{spot}(\omega-\mu)+\delta(\omega)(p^{spot}(\omega)-K)-q\Delta,\\
%\pi^{total}_P&:=&\pi_P+V_P\\
%&=& p^{spot}(\omega)(\mu-\omega)+\delta(\omega)(K-p^{spot}(\omega))+q\Delta,
%\end{eqnarray*}
%where
%\begin{equation*}
%p^{spot}(\omega) = \left\{ \begin{array} {ll}c_P \,\,&\,\, \text{if}\,\, \omega \in [\mu-\sqrt{3}\sigma,\mu),\\ 0\,\, &\,\,\text{if}\,\, \omega \in [\mu,\mu+\sqrt{3}\sigma]\end{array}\right.
% \end{equation*}


\iffalse



\subsubsection{Wind Power Producer} In the forward stage (at $t=0$), the wind power owner has to choose the amount of flexibility $\Delta$ to buy, given the option price and the strike price $(q,K)$ from the peaker generator owner. That is, he needs to choose his demand curve $\Delta(q,K)$ that maximizes his expected valuation of the swing option $\mathbb{E}_{\omega}[V_W(\omega)]$ (for this paper, we assume that all participants are risk-neutral). Assuming that he has the right conjecture on the spot price, his valuation function is 
\begin{equation*}
V_W(\omega) = \left\{ \begin{array} {ll}\delta(\omega)(c_P-K)-q\Delta\,\,&\,\, \text{if}\,\, \omega \in [\mu-\sqrt{3}\sigma,\mu),\\ -K\delta(\omega)-q\Delta\,\, &\,\, \text{if}\,\, \omega \in [\mu,\mu+\sqrt{3}\sigma].\end{array}\right.
 \end{equation*}

Note that when $\omega \in [\mu-\sqrt{3}\sigma,\mu)$, with a certainty equivalent dispatch, the wind power producer is exposed to negative payments as $\sigma$ grows. With the swing option, if $c_P\geq K$, he can exercise his right to purchase in real-time at strike price $K$ and increase his payment. To provide an incentive for the wind power producer to participate in this swing option and to avoid trivial cases, it is needed that $c_P\geq K+q$ (otherwise he will simply not purchase any flexibility $\Delta$), and we assume that this condition holds for the remaining of this example. In this case, when $\omega \in [\mu-\sqrt{3}\sigma,\mu)$, the wind power producer will find it beneficial to exercise all his right and choose $\delta(\omega)=\Delta$. On the other hand, when $\omega \in [\mu,\mu+\sqrt{3}\sigma]$, he will have no incentive to use his swing option in real-time, and he can set $\delta(\omega)=0$. Note that this is the set of scenarios at which there is a high availability of wind power, and the wind power producer is making profits. Taking these considerations into account, the valuation function becomes 
\begin{equation*}
V_W(\omega) = \left\{ \begin{array} {ll}\Delta(c_P-K-q)\,\,&\,\, \text{if}\,\, \omega \in [\mu-\sqrt{3}\sigma,\mu),\\ -q\Delta\,\, &\,\, \text{if}\,\, \omega \in [\mu,\mu+\sqrt{3}\sigma],\end{array}\right.
 \end{equation*}
which leads to 
\begin{eqnarray*} \mathbb{E}_{\omega}[V_W(\omega)]&=&\frac{\Delta(c_P-K-q)\sqrt{3}\sigma}{2\sqrt{3}\sigma}+\frac{-q\Delta\sqrt{3}\sigma}{2\sqrt{3}\sigma}\\
&=&\frac{\Delta(c_P-K-2q)}{2}.
\end{eqnarray*}
Thus, if the wind power producer receives $(q,K)$ such that $c_P\geq K+2q$, he is motivated to buy flexibility $\Delta^*$. Note that since the wind power producer will only exercise his option when $\omega \in [\mu-\sqrt{3}\sigma,\mu)$, and because $\overline{g}_W(\omega)=\omega$, in real-time, he can only sell up to $\omega=\mu$. Thus, he needs not to buy too much flexibility that he cannot sell in real time, and hence  $\Delta^*$ cannot exceed $\mu$. Taking these points into account, maximizing his expected valuation leads to $$\Delta^* = \left\{ \begin{array} {ll}\mu\,\,&\,\, \text{if}\,\, c_P\geq K+2q,\\ 0\,\, &\,\,\text{otherwise.}\end{array}\right.$$

\subsubsection{Peaker Generator Owner}

As an option seller, he needs to choose his supply curve $(q(\Delta),K(\Delta))$ at the forward stage $t=0$. Assuming that he has the right conjecture on the spot prices, the valuation of the swing option for the peaker plant is 
\begin{equation*}
V_P(\omega) = \left\{ \begin{array} {ll}\delta(\omega)(K-c_P)+q\Delta\,\,&\,\, \text{if}\,\, \omega \in [\mu-\sqrt{3}\sigma,\mu),\\ K\delta(\omega)+q\Delta\,\, &\,\, \text{if}\,\, \omega \in [\mu,\mu+\sqrt{3}\sigma].\end{array}\right.
 \end{equation*}

The real-time exercise amount $\delta(\omega)$ is unknown to the option seller. Since $c_P\geq K+q$, the multiplicative term of $\delta(\omega)$ is negative for $\omega\in [\mu-\sqrt{3}\sigma,\mu)$. Assuming the worst-case scenario, the peaker plant perceives $\delta(\omega)$ as $\Delta$ in this case. When $ \omega \in [\mu,\mu+\sqrt{3}\sigma]$, his worst case-scenario is to perceive $\delta(\omega)=0$. This implies that 
\begin{equation*}
V_P(\omega) = \left\{ \begin{array} {ll}\Delta(K-c_P+q)\,\,&\,\, \text{if}\,\, \omega \in [\mu-\sqrt{3}\sigma,\mu),\\ q\Delta\,\, &\,\, \text{if}\,\, \omega \in [\mu,\mu+\sqrt{3}\sigma].\end{array}\right.
 \end{equation*}
 
Under risk-neutrality, the peaker power plant aims to choose $(q,K)$ that maximize his expected valuation $\mathbb{E}_{\omega}[V_P(\omega)]$, for an exogenous $\Delta$. Note that 
\begin{eqnarray*} \mathbb{E}_{\omega}[V_P(\omega)]&=&\frac{\Delta(K-c_P+q)\sqrt{3}\sigma}{2\sqrt{3}\sigma}+\frac{q\Delta\sqrt{3}\sigma}{2\sqrt{3}\sigma}\\
&=&\frac{\Delta(K-c_P+2q)}{2},
\end{eqnarray*}
and to maximize the expected valuation he needs to select $(q,K)$ such that $c_P\leq K+2q$. But, it is needed that $c_P\geq K+q$ to avoid the trivial case at which the option buyer has no incentive to buy any flexibility $\Delta$ at all. Thus, with $\Delta$ being exogenous, the peaker plant chooses $(q^*,K^*)$ such that \begin{equation} K^*+q^* \leq c_P \leq K^*+2q^*.\end{equation}


\subsubsection{How is the swing option helping both participants?}
To elaborate on the benefits for the option buyer and the option seller, we let \begin{equation}c_P = K^*+2q^*. \end{equation}
Note that at this condition both the wind power producer and the peaker plant have an incentive to participate in the swing option. Particularly, at the above equality the wind power producer has an incentive to purchase $\Delta^*=\mu$. We note that with the above equality we have $$ \mathbb{E}_{\omega}[V_W(\omega)]= \mathbb{E}_{\omega}[V_P(\omega)]=0.$$

At $t=1$, if the realized scenario is such that the wind power producer is exposed to negative payments $\omega\in[\mu-\sqrt{3}\sigma,\mu)$, his valuation of the swing option is 
\begin{eqnarray*}
V_W(\omega)&=&\delta^*(\omega)(c_P-K^*-q^*)\\
&=&\Delta^*(c_P-K^*-q^*)\\
&=&\mu(c_P-K^*-q^*)=\mu q^*\geq0,
\end{eqnarray*}
and hence it is guaranteed that the volatility in payments reduce under high uncertainty, precisely, $$\pi^{total}_W\geq\pi_W.$$ Although the wind power producer reduces his volatility in payments. Under high uncertainty, it is still possible that he will be exposed to negative total payments. To elaborate, suppose that an extreme scenario is realized $\omega=\mu-\sqrt{3}\sigma$. Upon simple substitutions, the total payment becomes $$\pi^{total}_W=c_B\mu-c_P\sqrt{3}\sigma+\mu q^*,$$which can be negative as $\sigma$ grows. We can see that $\pi^{total}_W\geq0$ if and only if $$\sigma \leq \frac{\mu(q^*+c_B)}{\sqrt{3}c_P}.$$ On the other hand, in the certainty equivalent dispatch, it is needed that $$\sigma \leq \frac{\mu c_B}{\sqrt{3}c_P}$$ to guarantee that $\pi_W\geq0$. So, adding the flexibility results in a more relaxed upper bound on $\sigma$.

For the peaker plant, his valuation for a realization $\omega\in[\mu-\sqrt{3}\sigma,\mu)$ is \begin{eqnarray*}
V_P(\omega)&=&\Delta^*(K^*-c_P+q^*)
\\&=&-\mu q^*\leq0.\end{eqnarray*}
 
 Thus, although the volatility in payment for the wind power producer was reduced, the valuation of the peaker plant means he is worse-off when $\omega \in [\mu-\sqrt{3}\sigma,\mu)$. However, he had an incentive to participate and was compensated by $q\Delta$ at $t=0$. Furthermore, for some other scenarios, he can be better-off, and we discuss such cases next.
 
 Now, suppose that $\omega \in [\mu,\mu+\sqrt{3}\sigma]$. In this set of scenarios, there's a high availability of wind power and the wind power producer does not need to exercise his swing option, and we easily see that $$V_W(\omega)=-\mu q^* \,\, \text{and} \,\, V_P(\omega)=\mu q^*.$$
 
Thus, the peaker plant gains some profits $\mu q^*$ for selling the unused flexibility $\Delta^*=\mu$. We have the following proposition.

\begin{prop}
Under the condition $c_P\geq q+K$, both the wind power producer and the peaker power plant has an incentive to participate in the swing option. Furthermore, the following statements are true. 
\begin{itemize}
\item If the realized scenario $\omega\in[\mu-\sqrt{3}\sigma,\mu)$, the wind power producer is exposed to negative payments, and his participation in the swing option reduces his volatility of payments. 
\item If the realized scenario $\omega\in[\mu,\mu+\sqrt{3}\sigma]$, the wind power producer is not exposed to negative payments (the availability of wind power is high). So, the flexibility $\Delta$ will be unused and the peaker power plant gains profits $\mu q^*$.
\item $ \mathbb{E}_{\omega}[V_W(\omega)]+\mathbb{E}_{\omega}[V_P(\omega)]=0$.
\end{itemize}
\label{prop1}\end{prop}

\fi






